Collider Physics at HERA

From 1992 to 2007, HERA, the first electron-proton collider, operated at cms energies of about 320 GeV and allowed the investigation of deep-inelastic and photoproduction processes at the highest energy scales accessed thus far. This review is an introduction to, and a summary of, the main results obtained at HERA during its operation.

==> oldhch3.tex <==
%
%> 3. Proton Structure Functions             10          MK
\subsection{Introduction}
%
The scattering amplitude for electron-proton scattering is a product
of lepton and hadron currents times the propagator characteristic
for the exchanged particle, a photon or $Z_0$ in neutral current scattering
or a $W^{\pm}$ in charged current scattering. The inclusive scattering
cross section therefore is given by the product of two tensors,
\begin{equation}
\frac{d^2\sigma}{dxdQ^2} = \frac{2 \pi \alpha^2}{Q^4 x} 
\sum_j{\eta_j L_j^{\mu \nu} W_j^{\mu \nu}},
\end{equation} \label{siglw}
where $j$ denotes the summation over $\gamma$, $Z_0$ exchange
and their interference, for NC, or $j=W^+$ or $W^-$, for CC. The leptonic tensor
 $L_j^{\mu \nu}$ is related to the coupling of the electron with the
exchanged boson, containing the electromagnetic or the weak couplings,
as the vector and axial vector quark-$Z_0$ couplings, $v_q$ and $a_q$,
in the NC case.  This leptonic part of the cross
section can be calculated exactly in the standard electroweak $U_1 \times SU_2$
theory.  The hadronic tensor, however, describing the interaction of
the exchanged boson with the proton, can only be reduced to a sum of
structure functions, $F_i(x,Q^2)$, but not be fully calculated.
Basic conservation laws reduce the number of structure functions
in unpolarised $ep$ scattering to $i=1-3$.
In perturbative QCD the structure functions are related to 
parton distributions  $P$ $via$ coefficient functions $C$
%
\begin{equation}
 [F_{1,3},F_2] = \sum_i{\int_0^1{[1,z]\frac{dz}{z} C_{1,2,3}(\frac{x}{z},\frac{Q^2}{\mu_r^2},
 \frac{\mu_f^2}{\mu_r^2},\alpha_s(\mu_r^2)) \cdot P_{i}(z,\mu_f^2,\mu_r^2)}},
\end{equation} \label{factor}
%
where $i$ sums the quark $q$, anti-quark $\overline{q}$ and gluon $g$ contributions
and $P_i(x)$ is the probability of the parton of type $i$ to carry a fraction $x$
of the proton's longitudinal momentum. 
The coefficient functions are  exactly calculable
but depend on the factorisation and renormalisation scales $\mu_f$ and 
$\mu_r$. The parton distributions are not calculable but have to be
determined by experiment. A general factorisation
theorem, however, has proven them to be universal, i.e. to be independent of 
a certain type of hard scattering process. This makes 
deep inelastic lepton-nucleon scattering to be a
most fundamental process: the parton distributions in the proton
are measured best with a lepton probe and may be used
to predict hard scattering cross sections as at the LHC.
The parton distributions  are derived 
from measurements of the structure functions in NC and CC scattering,
as is discussed below.

In perturbative QCD  the parton distributions $P(x,Q^2_0)$, determined
at  an initial value $Q^2_0$, can be evolved  further in $Q^2$ using 
a system of coupled integro-differential equations
%
\begin{equation}
DGLAP,
\label{dglp}
\end{equation} 
%
which was 
introduced independently by Dokshitzer~\cite{yuri}, Gribov and 
Lipatov~\cite{griblip}
and by Altarelli and Parisi~\cite{altpar}.  From $\chi^2$ comparisons
of these QCD predictions with data, 
the quark and gluon momentum  distributions and
the strong coupling constant \amz can be determined.


The equations \ref{dglp} can be applied in 3rd order (NNLO) perturbation 
theory due to recent major progress in pQCD\,\cite{moch}. Most of
the parton distribution analyses, as those presented subsequently,
are still done in NLO. The next order will be important to match the
still increasing accuracy of further DIS measurements from H1 and ZEUS.
In these analyses the dependence as of \amz on the chosen scales $\mu$
will be reduced significantly. 

The HERA data are at sufficiently high $Q^2$ at
large $x$ such that power corrections, higher twists, $\propto Q^{-2}$
can be neglected. They extend to such low values of $x$, however,
that issues as to whether the evolution equations need to be modified
to include $\ln 1/x$ terms are under investigation, for
many years \cite{lowxcoll}, see section\,\ref{sec:lowx}. 
Besides attempts to replace the DGLAP equations by different
equations~\cite{bfkl,ccfm}, corresponding to modified rules of multi-gluon
emission at low $x$, the effects have also been investigated of
their modification with
a resummation of small $x$ logarithms \cite{ball}. For the
resolution of these questions
an increase in energy beyond HERA, as is considered with the LHeC\,\cite{lhec},
is very desirable in order to reach even lower $x$ and to perform
such investigations in a region of large enough $Q^2$ where \as is small.

The following sections describe the structure function formalism,
present important NC and CC measurements ending with a brief
overview on the most important pQCD analyses performed by ZEUS
and H1 to examine the partonic content of the proton.



\subsection{Structure Functions and Parton Distributions}
%HERA, the highest energy DIS laboratory, has covered a
%wide range in $x$ and $Q^2$ unaccessible hitherto.
%With accurate measurements of
%NC and CC processes using electron and positron beams, a 
%unique set of cross sections could be measured which allows a rather
%complete set of parton distributions to be derived.
%
The neutral  current deep inelastic ep scattering cross section, at tree level,
is given by a sum of generalised structure functions
according to 
%                                                                               
\begin{eqnarray} \label{ncsi}     
 \sigma_{r,NC} =\frac{d^2\sigma_{NC}}{dxdQ^2} \cdot \frac{Q^4 x}{2\pi \alpha^2 Y_+}                                                     
% \sigma_{r,NC} = \sigma_{r,0} + \sigma_{r,\gamma Z} + \sigma_{r,ZZ} &=&                   
  =            {\bf F_2} + \frac{Y_-}{Y_+} {\bf xF_3} -\frac{y^2}{Y_-} {\bf F_L}                      
% \sigma_{r,CC} = \sigma_{r,WW} &=&                                                  
%              {\bf W_2} + \frac{Y_-}{Y_+} {\bf xW_3}                                    
\end{eqnarray}                                                                  
%                                                                               
where the electromagnetic coupling, the photon              
propagator and a helicity factor are absorbed 
in the definition of a reduced cross section $\sigma_r$, and $Y_{\pm}=1 \pm (1-y)^2$.                                                                              
The functions ${\bf F_2}$ and  ${\bf xF_3}$ occurring in eq.(\ref{ncsi}) 
depend on the lepton beam charge and                  
polarization ($P$) and on the electroweak parameters,                     
e.g. on the weak boson masses  ($M_Z,~M_W$) and
the fine-structure constant  $\alpha$, as~\cite{klri}:                                                                       
%                                                                               
\begin{eqnarray} \label{strf}                                                   
 {\bf F_2^ \pm} &=& F_2 + \kappa_Z(-v_e \mp P a_e) \cdot F_2^{\gamma Z} +                      
  \kappa_Z^2 (v_e^2 + a_e^2 \pm 2 P v_e a_e) \cdot F_2^Z \nonumber \\                     
 {\bf xF_3^ \pm} &=&  \kappa_Z( \pm a_e + P v_e) \cdot xF_3^{\gamma Z} +                       
  \kappa_Z^2( \mp 2 v_e a_e - P (v_e^2+a_e^2)) \cdot xF_3^Z                                   
\end{eqnarray} 
%                                                                               
  with 
  $\kappa_Z(Q^2) =   Q^2 /[(Q^2+M_Z^2)(4\sin^2 \Theta \cos^2 \Theta)]$ 
and the weak mixing angle     $\sin^2  \Theta=1 -M^2_W /M^2_Z$.
In the hadronic tensor  decomposition~\cite{derman} the structure                                         
                    functions  are well defined                          
quantities, independently of the parton model. In the $QPM$  
the longitudinal structure function is zero\,\cite{cgross} and the 
two other functions are given by the sums and differences of
quark ($q$) and anti-quark ($\overline{q}$) distributions as                                                                               
%                                                                               
\begin{eqnarray} \label{ncfu}                                                   
  (F_2, F_2^{\gamma Z}, F_2^Z) &=&x \sum (e_q^2, 2e_qv_q, v_q^2+a_q^2)(q+\bar{q})            
                                 \nonumber \\                                   
  (xF_3^{\gamma Z}, xF_3^Z) &=& 2x \sum (e_qa_q, v_qa_q) (q-\bar{q}).                         
\end{eqnarray} 
%
where the sum extends over all up and down type quarks
and $e_q =e_u,e_d$ denotes the electric charge of up- or
down-type quarks. The vector and axial vector weak couplings of the fermions
($f=e,u,d$) to the $Z_0$ boson in the standard electroweak model
are given by
%
\begin{equation} \label{va}
 v_f= i_f - e_f 2 \sin^2 \Theta ~~~~~ a_f=i_f
 \end{equation}
%
 where   $e_f = -1,2/3,-1/3$ 
 and $i_f=I(f)_{3,L}=-1/2,1/2,-1/2$ denotes the
 left-handed weak isospin charges, respectively. Thus the vector coupling of the
 electron, for example, is very small, $v_e=-1/2 + 2 \sin^2 \Theta \simeq 0$
 since the weak mixing angle is roughly equal to 1/4. With a famous
 experiment~\cite{prescott}
  in polarised electron-nucleon scattering at very low $Q^2$
 it was observed that $a_e \simeq -1/2$ which did prove the absence of
 right-handed weak currents in the available energy range and thus the
validity of the most simple weak doublet structure in the now called
standard electroweak theory~\cite{GWS}.

Out of the 8 structure functions entering in eq.\,\ref{ncsi} four have been
accessed at HERA.  At low $Q^2$ the cross section is determined 
by $F_2$ and $F_L$, which at HERA is not small: it is measured at low $x$
where the gluon density is large, see below, leading to a rather
large value of $F_L$ as compared to previous fixed target measurements
at much larger $x$.

At low $Q^2$ and low $y$ the reduced cross section 
to very good approximation is given by $\sigma_r = F_2(x,Q^2)$. Indeed
most of the accurate knowledge  on the proton structure, at low $x$
from HERA and at large $x$ from fixed target experiments,
is due to precision measurements of $F_2$. At high $y > 0.5$ a sizeable
contribution to $\sigma_{r,NC}$ is made by $F_L$. In the DGLAP
approximation of perturbative QCD, to
lowest order, the longitudinal structure function is given by \cite{am}
%
\begin{equation}
        F_L(x) = \frac{\alpha_s}{4 \pi} x^2
        \int_x^1 \frac{dz}{z^3} \cdot \left[ \frac{16}{3}F_2(z) + 8
        \sum e_q^2 \left(1-\frac{x}{z} \right) zg(z) 
        \right]
\label{altmar}
\end{equation}
%
which at low $x$ is dominated by the gluon contribution, see below. 
Access to $F_L$ requires a variation of the beam energy
in order to remove the dominant $F_2$ contribution
to $\sigma_{r,NC}(x,Q^2;s) = F_2(x,Q^2) -y^2 F_L(x,Q^2)/Y_+$
and obtain $F_L$ as the slope in $y^2/Y_+$  at  fixed $x$ and $Q^2$,
as $y=Q^2/sx$.


Two further structure functions can be accessed with 
cross section asymmetry measurements
in which the charge or and the polarisation of the lepton beam are varied.
Both H1 and ZEUS have collected data samples of roughly 100\,pb$^{-1}$ 
of unpolarised
$e^+ p$ data and of similar luminosity in the two charge and opposite
helicity states, see table\,\ref{tabpoldata}
%
\begin{table}[htdp]\label{tabpoldata}
\begin{center}
\begin{tabular}{|l||l|l||l|l|l|l||l|}
\hline
exp & $e^+$ (0) & $e^-$ (0) & $e^+$ (0.33) & $e^+$ (-0.37) & $e^-$ (0.36) & $e^-$ (-0.26) & sum\\ 
\hline
H1  &  100 & 15& 95 & 75 & 46 & 103 & 432 \\
\hline
ZEUS  &  100 & 15& 70& 70& 70& 70 & 444\\
\hline
\end{tabular}
\caption{Integrated luminosity collected by H1 and ZEUS,
according to a specific data selection,
distinguished according to 
the beam charge and helicity (in parantheses) state. The unpolarised data
were taken in HERA I. While this review is written a significant
part of the polarised data, taken in the years 2004-2007,
is still being analysed.}
\end{center}
\end{table}
%


In the kinematic and luminosity reach of HERA the
electroweak asymmetry measurements access mainly the photon-$Z_0$
exchange part while the contributions, $\propto \kappa_Z^2$,
of the structure functions
$F_2^Z$ and $xF_3^Z$, which are due to pure $Z_0$ exchange, 
are rather negligible.
A charge asymmetry measurement,  with polarisation values $P_{\pm}$
of the $e^{\pm}$ beam, and $P_+ = -P_- =P$, thus
determines the following structure function combination 
%
\begin{equation} \label{casy}
 \sigma_{r,NC}^+(P) - \sigma_{r,NC}^-(-P) = -\kappa_Z 2 a_e [ P F_2^{\gamma Z} -  
 \frac{Y_-}{Y_+}xF_3^{\gamma Z}] 
\end{equation}
%
plus higher order terms. The amount of data in positron and
electron operation has been about balanced between positive and
negative helicity states, see Table\,\ref{tabpoldata}.
Thus the average polarisation may be adjusted to be zero
and the charge asymmetry becomes $\kappa_Z 2a_e xF_3^{\gamma Z}Y_-/Y_+$,
which  is a parity conserving quantity $\propto a_e a_q$.
This function, assuming symmetry between sea and antiquarks,
is a direct measure of the valence quarks, 
$xF_3^{\gamma Z} = 2 u_v + d_v$. It was measured 
for the first time in $\mu^{\pm}$ Carbon
scattering by the BCDMS Collaboration~\cite{xg3bcdms},
at large $x > 0.2$ and for $Q^2$ of about 50\,GeV$^2$. 
 Its salient feature at HERA is the ability to access valence quarks  in
the sea quark dominated region at low $x > 0.01$
and $Q^2 \simeq 1500$\,GeV$^2$, as is presented below.

A polarisation asymmetry measurement, for helicities $P_R$ and $P_L$,
according to  eqs.\,\ref{ncsi},\ref{strf}, determines a similar
combination of $F_2^{\gamma Z}$ and $xF_3^{\gamma Z}$
%
\begin{equation} \label{pasy}
\frac{ \sigma_{r,NC}^{\pm}(P_R) - \sigma_{r,NC}^{\pm}(P_L)}{P_R -P_L} 
 = \kappa_Z    [ \mp a_e F_2^{\gamma Z} +  \frac{Y_-}{Y_+} v_e xF_3^{\gamma Z}]
% \simeq  \mp \kappa_Z  a_e G_2 
\end{equation}
%
neglecting again the pure $Z$ exchange terms. The second term is 
a small correction only since the vector coupling is small, as is 
$Y_-=1-(1-y)^2$ in most of the kinematic range at HERA. 
The product $a_e F_2^{\gamma Z}$ is proportional to 
combinations $a_e v_q$ and thus
a direct measure of parity violation at very small distances,
~$10^{-18}$\,m, as are probed with electroweak cross section
measurements at HERA. 


The asymmetry 
% 
\begin{equation} \label{apm}
A^\pm = \frac{2}{P_R-P_L} \cdot \frac{\sigma_{NC}^{\pm}(P_R) -\sigma_{NC}^{\pm}(P_L)}
                          {\sigma_{NC}^{\pm}(P_R) +\sigma_{NC}^{\pm}(P_L)}
\end{equation}
to a very good approximation measures the structure function ratio  
\begin{equation}  \label{fgf}                                 
        A^\pm      
%        \simeq  \mp \kappa   a_e \frac{F_2^{\gamma Z}}{(F_2 + \kappa
%         a_e Y_- xF_3^{\gamma Z}/Y_+)} 
         \simeq \mp  \kappa_Z a_e \frac{F_2^{\gamma Z}}{F_2}.
\end{equation}
Thus $A^+$ is expected to be positive and about equal to $-A^-$.
 At large $x$  this asymmetries measure 
the $d/u$ ratio of the valence quark distributions according to
\begin{equation} \label{doveru} 
           A^\pm   \simeq  \pm  k \frac{1+d_v/u_v}{4+d_v/u_v}.
\end{equation}
%

Defining a similarly 
reduced cross section for inclusive polarised charged current $e^{\pm}$ p
scattering  as
%
\begin{equation}
 \label{Rnc}
 \sigma_{r,CC} =  
  \frac{2 \pi  x}{Y_+ G_F^2}
 \left[ \frac {M_W^2+Q^2} {M_W^2} \right]^2
          \frac{{\rm d}^2 \sigma_{CC}}{{\rm d}x{\rm d}Q^2}
\end{equation}
%
one obtains a sum of structure functions, like in eq.\,\ref{ncsi}, as
\begin{eqnarray}
 \label{ccsi}
 \sigma_{r,CC}^{\pm}=
 \frac{1\pm P}{2}( W_2^\pm   \mp \frac{Y_-}{Y_+} xW_3^\pm - \frac{y^2}{Y_+} W_L^\pm)\,.
\end{eqnarray}
%
Here the Fermi constant 
$G_F$ is defined~\cite{hector} using the weak boson
masses, in very good agreement with $G_F$ determined
from the measurement of the muon lifetime~\cite{pdg}.  
In the QPM (where $W_L^\pm = 0$),
the structure functions  represent
lepton beam-charge dependent sums and differences
of quark and anti-quark distributions given by
%
\begin{eqnarray}
 \label{ccstf}
    W_2^{+}  =  x (\bU+D)\hspace{0.05cm}\mbox{,}\hspace{0.1cm}
  xW_3^{+}  =  x (D-\bU)\hspace{0.05cm}\mbox{,}\hspace{0.1cm} 
    W_2^{-}  =  x (U+\bD)\hspace{0.05cm}\mbox{,}\hspace{0.1cm}
 xW_3^{-}  =  x (U-\bD)\,.
\end{eqnarray}
%

Using these equations one finds
%
\begin{eqnarray}
 \sigma_{r,CC}^+ \sim x\bU+ (1-y)^2xD, ~~\\
 \sigma_{r,CC}^- \sim xU +(1-y)^2 x\bD . ~~
\end{eqnarray}
%
Combined with eq.\,\ref{strf}, which approximately reduces to
%
\begin{eqnarray} \label{f23ud}
\sigma^{\pm}_{r,NC} \simeq [c_u (U+\bU) +c_d(D+\bD)] + \kappa_Z [d_u(U-\bU) + d_d (D-\bD)] \nonumber \\
%F_2 = x (e_u^2 (U+\bU) + e_d^2 (D + \bD)] \hspace{0.05cm}\mbox{,}\hspace{0.1cm}
%xG_3 = x [e_u a_u (U -\bU) + e_d a_d (D -\bD)]
\mbox{with} \hspace{0.2cm} c_{u,d} = e^2_{u,d} + \kappa_Z (-v_e \mp P a_e) e_{u,d}v_{u,d} 
\hspace{0.2cm} \mbox{and} \hspace{0.2cm} d_{u,d} = \pm a_e a_{u,d} e_{u,d},
\end{eqnarray}
%
one finds that the NC and CC cross section measurements at HERA 
determine the complete set   $U$, $D$, $\bU$ and $\bD$,
i.e. the sum of up-type, of down-type and of their 
anti-quark-type distributions. 
Below the $b$ quark mass threshold,
these are related to the individual quark distributions as follows
%
\begin{equation}  \label{ud}
  U  = u + c    ~~~~~~~~
 \bU = \bu + \bc ~~~~~~~~
  D  = d + s    ~~~~~~~~
 \bD = \bd + \bs\,. 
\end{equation}
%
Assuming symmetry between seaquarks and antiquarks, 
the valence quark distributions result from 
\begin{equation} \label{valq}
u_v = U -\bU ~~~~~~~~~~~~~ d_v = D -\bD.
\end{equation}


%
Eq.\,\ref{f23ud} also illustrates that the vector and axial vector couplings
of up and down type quarks can be determined at HERA. As will be discussed
below, recent QCD fits have obtained quite remarkable results on joint
determinations of parton distributions and of the weak 
neutral current coupling constants of the up and down type quarks
\footnote{One notices that the underlying assumption here is that
all up as all down type quarks have the same couplings, e.g. $a_u=a_c$.}.
%
\subsection{Measurements}
%
The measurement of inclusive neutral current scattering cross sections
employs the unique signature of an isolated electron cluster above certain
minimum energy, of a few GeV, in the LAr/Spacal (H1) or the U/Sc (ZEUS)
calorimeters. In charged current scattering a large transverse momentum, summing 
over all hadronic final state particles, is required, e.g. $p_T(h) > 12$\,GeV.
The NC and CC scattering events are required to have an
interaction vertex within the nominal interaction region, $\pm ~35$\,cm 
using the central trackers and, on the trigger level, of $\pm ~2$\,ns for ZEUS,
since the time resolution of the ZEUS calorimeter
is suited to distinguish genuine $ep$ scattering from beam background outside
the interaction region. NC events, unlike CC events, are balanced in the transverse
plane. Therefore the hadronic calorimeter can be calibrated requiring the ratio
$p_T(e)/p_T(h)$ to be close to one. The preceding calibration of the
electromagnetic calorimeters is based on the double angle method,
see Sect.\,\ref{diskine}, and, for lower $Q^2 < 500$\,GeV$^2$ it uses also 
the kinematic peak method. The linearity of the energy scale determination
is adjusted and calibrated, as in the case of the H1 Spacal calorimeter,
with the reconstruction of the $\pi_0$ and the $J/\psi$ mass, and checked
with elastic Compton events. The alignment techniques employ the redundancy of the
tracking system and also a peculiarity of elastic Compton events which have to be
back-to-back in the transverse plane.

The basic measurement technique is to compare the reconstructed
event distributions with a complete Monte Carlo simulation.
Backgrounds are subtracted from the data, most importantly the
events due to photoproduction which often mimic a DIS signature while
the scattered electron escaped near the beam axis. At small scattered
electron energies, $E_e' > 2$\,GeV this background may well exceed
the genuine DIS contribution. Therefore, in some analyses the calorimetric 
electron identification is complemented by a track associated to
the calorimeter cluster. Extra efficiencies, as of the trigger condition
used to select the CC or NC events, are determined from the data
and used to correct the simulation.  Radiative corrections to the
tree level cross section in NC can be much reduced requiring
the energy momentum in the event to be conserved, i.e.
$E-p_z \simeq 2E_e$, see Sect.\,\ref{diskine}. 
The simulation is normalised to
the measured luminosity, which is known to within $1-2$\,\% at HERA 
using Bethe-Heitler scattering, $ep \rightarrow ep \gamma$. 
The cross section, binned according to detector resolution, is then 
determined as the ratio of the background subtracted number of
DIS events in data to the simulated events, each corrected for
the luminosity of the data sample and the simulation, respectively,
and multiplied by the DIS cross section inherent to the simulation.

With this technique, much more detailed in several aspects, since 1993
both ZEUS~\cite{allzeus} and H1~\cite{allh1} have published
about 10 papers each on the measurements of the NC and
CC cross sections. The first measurements, shown in Fig.\,\ref{f292},
were based on only 0.03\,pb$^{-1}$ of data, taken in 1992.
With these first measurements the rise of the proton structure
function \F towards low $x$ was discovered.
The rise towards low $x$ is in agreement with basic expectations on the
low $x$ (large $\omega$) asymptotic limit of QCD~\cite{classics74}
which, however, had not fixed the actual scale of when it would set in. The
fixed target data gave rise to many possible extrapolations towards 
low $x$, for example, classic Regge theory~\cite{donland} expected $F_2$
to continue to be flat at low $x$. The curve shown 
in Fig.\,\ref{f292} was the expectation of
a model\,\cite{grv91}, in which the parton distribtions were generated dynamically
and evolved from a very low scale $Q^2 \simeq 0.3$\,GeV$^2$
towards higher $Q^2$. In this approach a rise towards low $x$ was
indeed expected.
%
%
\begin{figure}[h]
\begin{center}
\includegraphics[height=7.6cm]{herafig1ch3.eps}
\caption{The very first measurements of H1 (solid points) and ZEUS (open points)
of the proton structure function $F_2(x,Q^2)$ based on the data
taken in 1992 shown as a function of Bjorken $x$. The HERA collider
is equivalent to a fixed target lepton proton beam experiment
of about 50\,TeV beam energy. The HERA experiments thus were able to
extend the kinematic range of the $F_2$ data provided by the
fixed target electron (SLAC) and muon (BCDMS, NMC) proton experiments
by two orders of magnitude into the by then unknown domain of low $x$.
The curve shows a result  of the so-called dynamic parton distribution
approach. }
\end{center}
\label{f292}
\end{figure}
%

With increasing luminosity and improving understanding of such
a measurement, the accuracy was increased from about 20\% in the
first data to 2\% from recent measurements.  The data of H1 and
ZEUS have been consistent and often in good agreement for the
various NC and CC cross section data. The so far best published
measurements of the reduced cross section at low $Q^2$ are
displayed in Fig.\,\ref{bins}.   The left plot demonstrates the
rise of the cross section 
from the rise of $F_2$ towards low $x$ in all bins of $Q^2$.
In the intermediate $Q^2$ 
range the cross section, $\sigma_{r} = F_2 -y^2F_L/Y_+$,
is observed to flatten or even turning over under the influence of the 
$F_L$ term at high $y$. Dedicated measurements and analyses
are being performed to extract $F_L$ as is discussed below.

A further dramatic observation on the behaviour of $F_2(x,Q^2)$
was its strong dependence at fixed $x$ on $Q^2$, see the right plot
Fig.\,\ref{bins}. Thus the very first observations of scaling,
the independence of $F_2(x,Q^2)$ on $Q^2$, has been confirmed
only for $x \simeq 0.2$ where it was first discovered at SLAC\,\footnote{
For rather accidental reasons the energy and angular range of the
SLAC $ep$ spectrometer was such that it did correspond to
$x \simeq 0.2$. Therefore the first observations of inelastic DIS\,\cite{taylor}
occured in  a region where the behaviour of $F_2$ could
rather directly be related to the quark interpretation of the proton structure.
Departures from this behaviour, which were expected in 
field theory,  were first observed at Fermilab \cite{fnal74}
and with more accurate data they could be shown subsequently
to be logarithmic in $Q^2$. This was a major success in the
process of finding Quantum Chromodynamics as the 
appropriate field theory for  quark-gluon dynamics.}.
 The H1 and ZEUS measurements illustrate the important
differences between the scaling violations at high $x$, where they
are caused by gluon bremsstrahlung, and at low $x$, where
they are mainly due to $q \overline{q}$ pair production
from photon-gluon fusion. The strong rise with $Q^2$ at low $x$
is a major discovery of HERA. 

Confrontation of the measurements
with the evolution equations \ref{dglp} leads to the result
that at low $x$ the quark contribution to the $\ln Q^2$ derivatives
is negligible. This has two consequences: the measurement
as presented in Fig.\,\ref{bins} (right) can be interpreted as
the observation of a very large gluon distribution $xg(x,Q^2)$
which at fixed $Q^2$ rises with $x$. Furthermore,
neglecting the quark part, see \,\cite{prytz},
one can infer from the second DGLAP equation that 
 $ xg(x,Q^2)  \propto  \exp{\sqrt{c~\ln T~\ln (1/x)}}$ with
 $T=\alpha_s(Q^2)/\alpha_s(Q^2_0)$   \cite{muel}
and get a valid estimate of $F_2$ and its behaviour in $Q^2$ and $x$.
Indeed one is thus able to obtain that \F rises towards low $x$
as $ a x^{-\lambda}$  with $\lambda \propto \sqrt{\ln T/\ln (1/x)}$.
The rise is thus expected to be stronger as $Q^2$ increases
as indeed is observed, see Fig.\,\ref{bins} left.
A numeric study of this behaviour was performed in \cite{knd}.
Apart from the numeric success of this and further studies,
see for example \cite{haidt}, one finds that the proton structure
at low $x$ differs qualitatively very much from the large $x$ limit:
while the latter is given by the valence quark behaviour, the
low $x$ region is dominated by the dynamics of the QCD vacuum, the gluons.
%
\subsection{Low $\bf x$ Physics}
%
The physics of low $x$ has been in the focus of much theoretical
and experimental activity which for space reasons can only
briefly be mentioned here:
\begin{itemize}
\item
The rise of $F_2$ towards low $x$ has been examined quantitatively
\cite{zeusrise,h1rise}, see Fig.\,\ref{rose}.
For $x < 0.01$, where the valence quarks have
a negligible role, the rise at fixed $Q^2$
may be expressed as $F_2 = C x^{-\lambda}$.
It has been measured that for $Q^2 > 3.5$\,GeV$^2$, i.e. in the
DIS region, the parameter $C$ is constant and
$\lambda = 0.048 \ln Q^2/\Lambda^2$
with $\Lambda = 0.29$\,GeV. At lower $Q^2$, the rise gets weaker
and $C$ becomes dependent on $Q^2$. This may be interpreted
as a change from the partonic behaviour, at larger $Q^2$,
to a hadronic behaviour \cite{dolal}
at lower $Q^2$, the transition taking place
at $Q^2 \simeq 1$\,GeV$^2$ corresponding to a resolution
distance of about 0.3\,fm. A crucial role in this observation
played the accurate data below 1 GeV$^2$
of the ZEUS Collaboration which were
obtained with a dedicated detector placed in electron beam
direction near the beam pipe, together with the precision
measurements   based on the central apparatus of H1 and ZEUS.
%
\item
At lowest $x$, corresponding to large $y$, the reduced cross section
departs from $F_2$ because of $F_L$.  The longitudinal structure function
is a further measure of the gluon distribution 
which is independent and complementary to  the derivative
$\partial F_2(x,Q^2) /\partial \ln Q^2$. A measurement 
of $F_L(x,Q^2)$ thus represents
a crucial test of QCD to high orders as had long been studied
experimentally~\cite{flexp} and theoretically~\cite{flthy}.
The importance of this test at HERA rests  also on the observation
that the determinations of the gluon density at low $x$ and $Q^2$
are not constrained well because of the lack of range and the
uncertainties of the measurements of  $\partial F_2(x,Q^2) / \partial \ln Q^2$.
During the last 4 months of its operation, HERA was operated at
reduced proton beam energies, and data samples of 13\,pb$^{-1}$
at 460\,GeV and of 7\,pb$^{-1}$ at 565\,GeV were collected
both by ZEUS and by H1.
These should allow a clear separation of the contributions of $F_2$
and $F_L$ as is illustrated in Fig.\,\ref{rose}. This measurement
is particularly difficult because at high $y \simeq 1 -E_e'/E_e$
the scattered electron energy is rather small, $E_e' \geq 2.7$\,GeV
in the data analyses. At such low energies the genuine
DIS electron signal is mimiced by hadronic energy depositions
as are frequently due to photoproduction processes posing 
extra difficulties to trigger and electron identification.
Since the luminosity behave as $L \propto E_p^2$, a reduction
to half the energy requires 4 times longer running. A preciser 
measurement for practical reasons will thus be restricted
to the lower $Q^2$ region. As this paper is being written, both the
ZEUS and H1 Collaborations analyse the low energy run data and
results are  much awaited. These will complement and  
perhaps validate previous attempts by
the H1 Collaboration which were designed to
extract information on $F_L$ from
the reduced cross section under certain assumptions on the
behaviour of $F_2$, see \cite{flh1}.
%
\begin{figure}[h]
\begin{center} 
\includegraphics[height=5.1cm]{herafig2ach3.eps}
\includegraphics[height=6.cm,angle=90.]{herafig2bch3.eps}
\caption{Left: Rise of $F_2$ versus $x$ as a function of $Q^2$, see
text. Note that with $Q^2$ also $x$ varies, roughly as
$x \sim Q^2/0.1 s$ GET COMBINED H1-ZEUS PLOT. Right:
Simulated measurement of the reduced cross
section $\sigma_{r,NC} = F_2 -f(y) F_L$ at $Q^2=10$\,GeV$^2$
as is anticipated with H1. The inner error bars are the statistical 
uncertainty and the full error bars are the expected
systematic and statistical uncertainties added in quadrature.
The two structure function contributions
 can be measured  as slope ($F_L$) and intercept ($F_2$)
of $\sigma_r$ versus $f(y)=y^2/[1+(1-y)^2]$. 
}
\label{rose}
\end{center}
\end{figure}
%
\item
At low $x$ the view on the $ep$ interaction may be changed:
instead of using the parton picture  and the infinite momentum
frame\,\cite{feynman} one may  consider the virtual photon
proton interaction in the proton restframe. The virtual 
photon disintegrates long before interacting with the proton,
at a coherence length $\propto 1/x$ apart, into a dipole
of quark and antiquark which hits the proton. This picture, 
originally considered in \cite{gribov} and turned 
into the colour diploe model (CDM) in \cite{cdm}, has received much
attention over the years of HERA's existence \cite{cdmrev} because of its
simplicity and universality. The CDM is able to provide predictions,
using a phenomenological ansatz for a hard scattering cross 
section, for a variety of cases, as for the structure functions
$F_2$, $F_L$ but as well for the diffractive and heavy quark
structure functions, which are introduced below.  The strict
relations between these predictions lead to crucial tests
of the validity of this approach \cite{nachtcdm}, results of
which can still be expected at HERA. The CDM model
fundamentally does not distinguish between the partonic or hadronic
behaviour of the proton and thus is applicable for large as well
as very small values of $Q^2$ in DIS. It is to be also noted that
the transverse size of the dipole is $2/\sqrt{Q^2}$, thus with variing
the momentum transfer one is also able to probe the transverse
extension of the proton. Most noteably at HERA the transverse
size of gluons was measured for the first time, see \cite{gluontran}
CHECK
%
\item
%
unintegrated, f2c, final states ...
\end{itemize}
 
\subsection{Measurements at High $\bf Q^2$}

\begin{figure}[h]
\begin{center}
\includegraphics[height=7.6cm]{herafig3ach3.eps}
\includegraphics[height=7.6cm]{herafig3bch3.eps}
%\includegraphics[height=7.6cm]{bwncepa.eps}
%\includegraphics[height=7.6cm]{bwbins.eps}
%\epsfig{file=bins1.eps,scale=0.8}
\caption{Deep inelastic neutral current $e^+p$ scattering cross
 section measurements, from the HERA I data taking period,
  as a function of $x$ in different $Q^2$
 intervals (left) and  
 for  three selected $x$ bins as a function of $Q^2$ (right).
  Open points: H1, open squares: ZEUS.
    The error bars show the total uncertainty.
    The curves are NLO QCD fits as performed 
   by H1 and ZEUS to their own data. The flattening of the curves
   for the two lower $x$ values at large $Q^2$ is due to the effect of $F_L$.
    At $x = 0.25$ the data and the curves decrease visibly for
     $Q^2$ above a few 1000\,GeV$^2$. This effect results from
      the effect of the $\gamma Z$ interference which reduces
       the cross section in positron-proton scattering at high $Q^2$,
        cf. eq.\,\ref{strf}
        , $\propto a_e xF_3^{\gamma Z}$ with $a_e=-1/2$.}
\label{bins}
\end{center}
\end{figure}






\begin{figure}[htbp]
\begin{center}
%\epsfig{file=scal1.eps,scale=0.8}
\includegraphics[height=7.6cm]{herafig4ach3.eps}
\includegraphics[height=7.6cm]{herafig4bch3.eps}
%\includegraphics[height=7.6cm]{bwscal.eps}
%\includegraphics[height=7.6cm]{bwncepb.eps}
\caption{ Deep inelastic neutral current $e^+p$ scattering cross
 section  data from the HERA I data taking period. Left:
 HERA data versus $Q^2$ for different $x$. The HERA collider
 measurements are consistent with former DIS fixed target
 measurements but considerably extend the kinematic range
 in $Q^2$ and $x$. Right: NC cross section data
 versus $x$ in different intervals of $Q^2$.  
 The curves are NLO QCD fits as performed by H1 and ZEUS
 to their own data.}
\label{scalscal}
\end{center}
\end{figure}




\begin{figure}[htbp]
\begin{center}
%\epsfig{file=ccep1.eps,scale=0.8}
\includegraphics[height=7.6cm]{herafig5ach3.eps}
\includegraphics[height=7.6cm]{herafig5bch3.eps}
%\includegraphics[height=7.6cm]{bwccep.eps}
%\includegraphics[height=7.6cm]{bwccem.eps}
\caption{ Deep inelastic charged current $e^{\pm}p$ scattering cross
 section  for  $Q^2$ between $300$ and $30000$\,GeV$^2$,
 obtained from published by 
 H1 and ZEUS using data taken in HERA I. 
 The curves are NLO QCD fits as performed by H1 and ZEUS
 to their own data.}
\label{ccep}
\end{center}
\end{figure}






%
\subsection{Determinations of Parton Distributions and of $\bf \alpha_s$}
%
In QCD the deep inelastic lepton nucleon scattering cross section
appears as a convolution of parton distributions with theoretically
well defined coefficient functions. Inclusive DIS is thus free of
extra nonperturbative parameters which complicate the QCD
interpretation of semiinclusive data. The combination of proton and
deuteron structure function data has long been recognized to be 
particularly well suited for the measurement of the strong coupling
constant \as~\cite{vm} and of the gluon distribution. 
 
A NLO QCD fit to the cross section data of this experiment and of
muon scattering experiments was performed 
in the $\overline{MS}$ renormalization scheme using the
DGLAP evolution equations~\cite{dglap} for three light flavours with the charm
contribution added according to 
the NLO calculation of the photon-gluon fusion
process \cite{lae2}. In the
one-photon exchange approximation the deep inelastic lepton nucleon
scattering cross section, Eq.\ref{sig},
is essentially determined by the proton and deuteron structure
functions $F_2^p$ and $F_2^d$.  These functions have the following
three-flavour decomposition
%
\begin{eqnarray}\label{f2p}
 F_2^p = \frac{5}{18} \cdot S + \frac{1}{6} \cdot D, \nonumber \\
 F_2^d = \frac{5}{18} \cdot S - \frac{1}{6} \cdot (s+\bs)
\end{eqnarray}
%
which is defined by two 
independent combinations of parton distribution functions
%
\begin{eqnarray}\label{sd}
  S = u + \bu + d + \bd + s + \bs  , \nonumber \\
  D = u + \bu - d - \bd - s - \bs
\end{eqnarray}
%
besides the strange quark contribution $s+\bs$. Here the symbols 
$q=u, d, s$ denote the parton distributions $x~q(x,Q^2)$. 
In the course of the QCD
analysis it turned out to be necessary to separate the valence parton
distributions $u_v$ and $d_v$ from the sea since the
parametrizations of the functions $S$ and $D$ otherwise
required too many conflicting parameters to describe the 
$x$ dependence of these effective parton distributions.
Thus the following combinations were used
%
\begin{eqnarray}\label{cp}
  V= u_v + d_v,  \nonumber \\
  B = \bu + \bd, \nonumber \\
  Q^+ = u + \bu - d - \bd.
\end{eqnarray}
%
Adopting the procedure of \cite{mrs} the strange contribution 
$s + \bs$ was coupled to the sea quarks using $s + \bs = (\bu + \bd)/2$ as
supported by the measurement of the strange sea quark distribution 
in \cite{neusea}.
  
 The consideration of $Z$ exchange
would require to introduce further combinations of parton
distributions~\cite{tr} which, however, could not be well determined
at the present accuracy level of the high $Q^2$
data~\cite{hiq}. Thus cross section data with $Q^2 > 2000$~\gv were not
included in this analysis. 


The input parton distributions $p= V, B, Q^+, g$ 
were parametrized at the starting scale $Q^{2}_{o}$ as follows:
%
\begin{equation}\label{para}
xp(x) = A_px^{B_p}(1-x)^{C_p}(1+D_{p}x+E_{p}\sqrt{x}).
\end{equation}
%
For the sum $V$ of valence quark distributions the quark
counting rule was used and the momentum sum rule was applied.

The fit was performed using an $x$ space program developed inside
the H1 collaboration~\cite{zopa}. 
The implementation of the NLO evolution was found 
to be in very good agreement~\cite{hwspro} with
independent programs, one of them being written in moment space.
Small departures from the results of the programs of the MRST
and CTEQ analysis groups were recently explained by
them~\cite{mrstcorr, cteqc}. 

The QCD analysis was based on
the reduced cross section, eq.\ref{sig}, and not only
its \F part, which did  avoids the introduction of $ad~hoc$
assumptions on \FL and allowed all data up to highest $y$
to be included  in the QCD analysis. The muon-proton 
and muon-deuteron DIS cross sections measured by the 
experiments BCDMS \cite{BCDMS} and NMC \cite{NMC}
were also used to constrain the high $x$ behaviour of the parton 
distributions. Target mass corrections were applied 
according to \cite{tarmas}.
The starting point of the evolution was chosen to be $Q_o^2 = 4$ 
GeV$^2$ and  data with $Q^2 \geq Q^2_{min}=4$~GeV$^2$
were included in the fit. 
 A cut was made to exclude BCDMS data in the
region sensitive to higher twists ($x > 0.5$ for $Q^{2} < 
15$~GeV$^{2}$).
For the standard fit values of $\alpha_s(M_Z^2)=0.118$ and $m_c=1.5$~GeV
were chosen. 

%
%\section{low-x, FL} \label{slowx}
%
\begin{figure}[htbp]
\begin{center}
%\epsfig{file=ncepa1.eps,scale=0.8}
%\includegraphics[height=9cm]{ncepa1.eps}
\caption{ Deep inelastic neutral current $e^=p$ scattering cross
 section  at low $Q^2$ and $x$
% for lower $Q^2$, $1.5 - 120$\,GeV$^2$,
 as obtained by
 H1 and ZEUS  from data taken in HERA I. 
 The curves are NLO QCD fits as performed by H1 and ZEUS
 to their own data, shown for $Q^2 \geq Q^2_{min}$ as chosen
 in the fit procedure. Note that there are data available for
 $Q^2$ below 1\,GeV$^2$, both from shifted vertex operation and from
 ZEUS also using a detector, $BPC$, near the beam pipe. 
 WOULD BE GOOD TO SHOW THEM PERHAPS VS W}
\label{ncepa}
\end{center}
\end{figure}
use h1 eoi for FL
% 

